Template-based Monocular 3D Shape Recovery using Laplacian Meshes

We show that by extending the Laplacian formalism, which was first introduced in the Graphics community to regularize 3D meshes, we can turn the monocular 3D shape reconstruction of a deformable surface given correspondences with a reference image into a much better-posed problem. This allows us to quickly and reliably eliminate outliers by simply solving a linear least squares problem. This yields an initial 3D shape estimate, which is not necessarily accurate, but whose 2D projections are. The initial shape is then refined by a constrained optimization problem to output the final surface reconstruction. Our approach allows us to reduce the dimensionality of the surface reconstruction problem without sacrificing accuracy, thus allowing for real-time implementations.

==> figs_accuracy.tex <==
%% -*- mode: latex; mode: reftex; mode: flyspell; mode: auto-fill; TeX-master: "top.tex"; -*-

%pf 23/01/13 Changed the order to make  it the same as in the description of the
%            datasets. 
%pf 23/01/13  The graphs that go  into negative territory are  weird. Please fix
%             this. 
\newcommand{\errheight}{3.5cm}
\begin{figure*}
  \centering
  \hspace{-2em}
  \begin{tabular}{cccc}
    \includegraphics[height=\errheight]{figs/ctrlchoice/capaper.pdf}            &
    \includegraphics[height=\errheight]{figs/ctrlchoice/siftextbanana12.pdf}        &
    \includegraphics[height=\errheight]{figs/ctrlchoice/siftextball2.pdf} & 
     \includegraphics[height=\errheight]{figs/ctrlchoice/sailscaled.pdf}          
\\ (a) &
    (b) & (c) & (d)
  \end{tabular}
% JÖ: The formulation in the caption what the bracketed numbers mean
% is a bit clumpsy but hopefully clear.
%pf 23/01/13 What do you do for the sail? 
\caption{{\bf   Comparative  accuracy   results   for  the   four  datasets   of
    Section~\ref{sec:datasets}.} {\bf  (a)} Paper {\bf  (b)} Banana
  leaf {\bf(c)}
  Ball.  {\bf (d)} Sail.  The ``Ours-manual'' green and white bars represent the
  accuracy of our Laplacian approach  using the manually selected control points
  of Fig.~\ref{fig:choosectrl}  and the ``Ours-optimized'' violet  and
  cyan ones represent
  those obtained using the optimized configurations. For comparison purposes, we
  draw the corresponding accuracy results obtained using a linear subspace model
  and the  approach of~\cite{Salzmann11a}, in  gray and blue  respectively. Each
  bracketed number  in the  legends is one  third of  the numbers of  degrees of
  freedom involved in each computation,  that is, the number of control vertices
  when using our Laplacian approach.}
  \label{fig:error3d}
\end{figure*}


==> figs_robustness_robustness.tex <==
\newcommand{\robustw}{0.43\linewidth}
\newcommand{\robusth}{0.33\linewidth}
\begin{figure*}[t]
\begin{center}
\begin{tabular}{cc}
 \includegraphics[width=\robustw, height=\robusth]{figs_robustness_ours_paper_mesh.pdf} \hspace{0.3cm} &
 \includegraphics[width=\robustw, height=\robusth]{figs_robustness_ours_paper_inlier.pdf} \\
 \includegraphics[width=\robustw, height=\robusth]{figs_robustness_ours_cushion_mesh.pdf} \hspace{0.3cm} &
 \includegraphics[width=\robustw, height=\robusth]{figs_robustness_ours_cushion_inlier.pdf} \\
 (a) \hspace{0.3cm} &(b)
 %\vspace{-.3cm}
\end{tabular}
\end{center}
\caption{Probability of  success as a function  of the number of  inlier matches
  and proportion of outliers, on the  x-axis and y-axis respectively.  The lines
  are level  lines of the probability  of success according to  the two criteria:
  (a) Probability of  having at least $90\%$ mesh vertices  reprojected within 2
  pixels of the solution (b) Probability of retrieving at least $90\%$ of inlier
  input  matches.  {\bf  Top row:}  paper  dataset.  {\bf  Bottom row:}  cushion
  dataset.}
\label{fig:robustness}
\vspace{-.2cm}
\end{figure*}


==> reconstruction.tex <==
%% -*- mode: latex; mode: reftex; mode: flyspell; mode: auto-fill; TeX-master: "top.tex"; -*-






